Compounding Effect of Harsh Climate and Societal Disruptions on Food Prices in Early Modern Europe

The complex interplay between famine, warfare, and climate constitutes a multifaceted and context-dependent relationship that has profoundly influenced human history, particularly in early modern Europe. This study advances the literature on climate-economy interactions by leveraging multi-scale statistical techniques to quantify the compounded effects of climate variability and socio-political factors on food prices, offering novel model-based insights into the historical dynamics of climate and economic systems. Using Canonical Correlation Analysis (CCA), we investigate the influence of temperature fluctuations and drought severity on food prices across 14 European cities from 1565 to 1785. Our findings confirm a persistent negative relationship between temperature and food prices over the long term, while the relationship between drought severity and price dynamics appears positive yet inconsistent. Extending our analysis to higher-frequency patterns, we demonstrate that cold anomalies are strongly associated with food price that caused large-scale famines of the 1590s and 1690s. Likewise, we show that the severe and consecutive droughts of 1634 to 1636, coinciding with the Thirty Years' War, significantly amplified food price volatility, illustrating how climatic shocks can compound socio-economic and political crises. Furthermore, we identify years characterized by the simultaneous occurrence of extreme cold and drought as periods of heightened price instability, underscoring the compounded impact of concurrent climatic stressors on food prices during the early modern period.

==> regs_cor_temp.tex <==

\begin{table}
\caption{Dep. Var. : Temperature/CPI Correlation}
\begin{center}
\begin{threeparttable}
\begin{tabular}{l c c c}
\hline
 & 10Y corr & 15Y corr & 20Y corr \\
\hline
famines & $-0.094 \; (0.012)^{***}$ & $-0.063 \; (0.010)^{***}$ & $-0.023 \; (0.008)^{**}$ \\
TY\_war & $-0.026 \; (0.013)$       & $0.005 \; (0.012)$        & $0.029 \; (0.010)^{**}$  \\
CPI     & $0.026 \; (0.022)$        & $-0.036 \; (0.017)^{*}$   & $-0.037 \; (0.016)^{*}$  \\
temp    & $-0.018 \; (0.010)$       & $-0.012 \; (0.008)$       & $-0.005 \; (0.007)$      \\
\hline
N       & $2828$                    & $2828$                    & $2828$                   \\
\hline
\end{tabular}
\begin{tablenotes}[flushleft]
\scriptsize{\item $^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$. \  Newey-West standard errors are clustered at the location level.}
\end{tablenotes}
\end{threeparttable}
\label{tab:regs_cor_temp}
\end{center}
\end{table}

